Blaze: Simplified High Performance Cluster Computing

MapReduce and its variants have significantly simplified and accelerated the process of developing parallel programs. However, most MapReduce implementations focus on data-intensive tasks while many real-world tasks are compute intensive and their data can fit distributedly into the memory. For these tasks, the speed of MapReduce programs can be much slower than those hand-optimized ones. We present Blaze, a C++ library that makes it easy to develop high performance parallel programs for such compute intensive tasks. At the core of Blaze is a highly-optimized in-memory MapReduce function, which has three main improvements over conventional MapReduce implementations: eager reduction, fast serialization, and special treatment for a small fixed key range. We also offer additional conveniences that make developing parallel programs similar to developing serial programs. These improvements make Blaze an easy-to-use cluster computing library that approaches the speed of hand-optimized parallel code. We apply Blaze to some common data mining tasks, including word frequency count, PageRank, k-means, expectation maximization (Gaussian mixture model), and k-nearest neighbors. Blaze outperforms Apache Spark by more than 10 times on average for these tasks, and the speed of Blaze scales almost linearly with the number of nodes. In addition, Blaze uses only the MapReduce function and 3 utility functions in its implementation while Spark uses almost 30 different parallel primitives in its official implementation.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> docs/introduction_old.tex <==

It has been a decade since the MapReduce paradigm~\cite{dean2008mapreduce, dean2010mapreduce,dean2006experiences} was firstly introduced by Google for simplified data processing on large computing clusters.


MapReduce and its improved variants~\cite{dean2008mapreduce, chambers2010flumejava, dean2010mapreduce, zaharia2010spark, zaharia2016apache,condie2010mapreduce,zaharia2008improving,goiri2015approxhadoop,afrati2010optimizing,li2015coded,ekanayake2010twister,he2008mars,bhatotia2011incoop} have significantly simplified parallel programs to make use of large computing clusters by
\begin{itemize}
    \item providing a high-level abstraction with powerful interface to users and
    \item taking care of the low-level operations, such as distributing workloads and communicating between machines.
\end{itemize}


This paradigm has been used in almost all major tech companies serving billions of users around the world, which was proved to be not only successful in practice but also inspiring for further development of computing cluster technologies. 

Although the computational efficiency of applications like processing crawled documents, web log requests tremendously benefit from the MapReduce paradigm, conventional MapReduce libraries cannot satisfy the increasing demanads of machine learning and data mining related tasks.
Several MapReduce-oriented libraries~\cite{bosagh2016matrix, meng2016mllib, shanahan2015large} have been further investigated to improve the performance in handling machine learning and data mining.
However, these libraries are developed solely based on one variant of MapReduce paradigm called Spark~\cite{zaharia2010spark, zaharia2016apache}, which has several severe limitations for machine learning and data mining applications. 

As shown in Fig.\ref{fig:mr}, MapReduce is a data processing paradigm where we first map each element of the input data to one or more key-value pairs using a map function and then reduce all the pairs with the same key by an associative reduce function to get a single key-value pair for each unique key. With appropriate design considerations, MapReduce operations can be stacked together to describe most cloud applications, from the search engine that we use everyday to advanced analysis procedures in professional business intelligence solutions. 
% MapReduce implementations, such as Hadoop and Spark, provide developers with well-encapsulated classes that are robust and scalable, so that developers can focus more on their applications. 
% At the time of this writing, MapReduce and its variants are being used in all the major tech companies, .

Although widely-used, most MapReduce implementations focus on their capability rather than the performance, which significantly reduces the performance in the applications of machine learning and data mining. 
Hadoop MapReduce stores all the intermediate results to persistence storage devices, which enables the system to handle extremely large datasets but meets serious runtime overhead. 
Spark provides in-memory MapReduce which can outperform Hadoop by one to two orders of magnitude; however, Spark imitates the original MapReduce pipeline that is specifically designed for spinning disks, which provides large room for performance optimization for applications that require intensive data processing and memory fitting.
For in-memory MapReduce, the bottleneck shifts from the disks to the amount of computation and the network communication. 
Our study tries to alleviate these new bottlenecks and build a highly-optimized MapReduce library from ground up.

The most important motivation of building Blaze is that we meet severe performance limitations when apply traditional MapReduce framework to quantum chemistry computations, which requires to solve for the lowest few eigenvalues of a sparse Hamiltonian matrix of size $10^{29} \times 10^{29}$, where we repeatedly process trillions of non-zero matrix elements deterministically and $10^{32}$ other non-zero matrix elements stochastically~\cite{li2018fast}. 
However, traditional MapReduce framework requires several months of computations for certain tasks, which is unendurable for real-world quantum chemistry applications.
Later a scientific computation tool with hand-optimized MapReduce called Arrow is born to meet the high demanding quantum chemistry, which is at least $10 \times$ faster than original MapReduce framework.
Although developed just a year ago, Arrow has already been running stably in several world-lead quantum chemistry research groups.

Based on the deep understanding of the quantum computing process with MapReduce, we find that similar framework with a few additional performance optimization can be used to numerous data mining and machine learning related tasks as well. 
Therefore, we factor out our MapReduce implementation, together with some other utility functions and distributed data containers into a standalone library called \texttt{\textbf{Blaze}}.

The contributions of this study are listed as follows:

\begin{itemize}

    \item Fast serialization is implemented so that we could achieve higher performance on encoding/decoding and obtain smaller sizes for encoded messages. This tremendously reduces the inter-node communication cost.
    \item Sort separation is introduced to remove the sort step from MapReduce as key orders are not important in many data mining applications. 
    The sort is replaced with a non-blocking distributed hash table that is designed specifically for data mining in MapReduce, which reduces the total time complexity of MapReduce from O(nlogn) to O(n). 
    For cases that key orders are important, native sort function or special parallel sorting libraries could be applied as well.
    \item Efficient eager function is introduced to perform simultaneous map and reduce, which enables streaming data processing. This not only reduces the memory requirement of MapReduce so that we can use in-memory MapReduce on larger datasets, but also lowers the burden of inter-node communication cost.
    \item We incorporate the improvements above as well as various small improvements and build Blaze, which is a blazing fast MapReduce library that can outperform Spark by 5x on common MapReduce tasks. 
    Similar to Spark, it also supports reusing working datasets for multiple MapReduce operations.
\end{itemize}
